Implementation of Analytical Jacobian and Chemical Explosive Mode Analysis (CEMA) in OpenFOAM

This report presents the implementation details of the chemical explosive mode analysis (CEMA), using analytical Jacobian formulation, into OpenFOAM.

==> Codes/controlDict <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       dictionary;
    location    "system";
    object      controlDict;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

application     icoFoam;

startFrom       startTime;

startTime       0;

stopAt          endTime;

endTime         0.5;

deltaT          0.005;

writeControl    timeStep;

writeInterval   20;

purgeWrite      0;

writeFormat     ascii;

writePrecision  6;

writeCompression off;

timeFormat      general;

timePrecision   6;

runTimeModifiable true;

functions
{
//    #include "surfaces"

    minMax
    {
        type            fieldMinMax;
        libs            (fieldFunctionObjects);
        fields          (p);
    } 
}
// ************************************************************************* //


==> Codes/lib_standard/chemistryModel/Make/options <==
EXE_INC = \
    -I$(LIB_SRC)/finiteVolume/lnInclude \
    -I$(LIB_SRC)/meshTools/lnInclude \
    -I$(LIB_SRC)/ODE/lnInclude \
    -I$(LIB_SRC)/transportModels/compressible/lnInclude \
    -I$(LIB_SRC)/thermophysicalModels/reactionThermo/lnInclude \
    -I$(LIB_SRC)/thermophysicalModels/basic/lnInclude \
    -I$(LIB_SRC)/thermophysicalModels/specie/lnInclude \
    -I$(LIB_SRC)/thermophysicalModels/functions/Polynomial \
    -I$(LIB_SRC)/thermophysicalModels/thermophysicalFunctions/lnInclude

LIB_LIBS = \
    -lfiniteVolume \
    -lmeshTools \
    -lODE \
    -lcompressibleTransportModels \
    -lfluidThermophysicalModels \
    -lreactionThermophysicalModels \
    -lspecie


==> Codes/tutorial/0/CH4 <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       volScalarField;
    location    "0";
    object      CH4;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

dimensions      [0 0 0 0 0 0 0];

internalField   nonuniform
#include"CH4.dat"
;

boundaryField
{
    inlet
    {
        type            fixedValue;
        value           uniform 0.0283654;
    }

    outlet
    {
        type            zeroGradient;
    }

    frontAndBack
    {
        type            empty;
    }
}

// ************************************************************************* //


==> Codes/tutorial/0/CO2 <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       volScalarField;
    location    "0";
    object      CO2;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

dimensions      [0 0 0 0 0 0 0];

internalField   nonuniform
#include"CO2.dat"
;

boundaryField
{
    inlet
    {
        type            fixedValue;
        value           uniform 0.0;
    }

    outlet
    {
        type            zeroGradient;
    }

    frontAndBack
    {
        type            empty;
    }
}

// ************************************************************************* //


==> Codes/tutorial/0/H2O <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       volScalarField;
    location    "0";
    object      H2O;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

dimensions      [0 0 0 0 0 0 0];

internalField   nonuniform
#include"H2O.dat"
;

boundaryField
{
    inlet
    {
        type            fixedValue;
        value           uniform 0.0;
    }

    outlet
    {
        type            zeroGradient;
    }

    frontAndBack
    {
        type            empty;
    }
}

// ************************************************************************* //


==> Codes/tutorial/0/N2 <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       volScalarField;
    location    "0";
    object      N2;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

dimensions      [0 0 0 0 0 0 0];

internalField   nonuniform
#include"N2.dat"
;

boundaryField
{
    inlet
    {
        type            fixedValue;
        value           uniform 0.7453246;
    }

    outlet
    {
        type            zeroGradient;
    }

    frontAndBack
    {
        type            empty;
    }
}

// ************************************************************************* //


==> Codes/tutorial/0/O2 <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       volScalarField;
    location    "0";
    object      O2;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

dimensions      [0 0 0 0 0 0 0];

internalField   nonuniform
#include"O2.dat"
;

boundaryField
{
    inlet
    {
        type            fixedValue;
        value           uniform 0.22631;
    }

    outlet
    {
        type            zeroGradient;
    }

    frontAndBack
    {
        type            empty;
    }
}

// ************************************************************************* //


==> Codes/tutorial/0/T <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       volScalarField;
    location    "0";
    object      T;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

dimensions      [0 0 0 1 0 0 0];

internalField   nonuniform
#include"T.dat"
;

boundaryField
{
    inlet
    {
        type            fixedValue;
        value           uniform 900;
    }

    outlet
    {
        type              zeroGradient;
    }

    frontAndBack
    {
        type            empty;
    }
}

// ************************************************************************* //


==> Codes/tutorial/0/U <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       volVectorField;
    location    "0";
    object      U;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

dimensions      [0 1 -1 0 0 0 0];

internalField   uniform (0 0 0);

boundaryField
{
    inlet
    {
        type            fixedValue;
        value           uniform (1.456 0 0);
    }

    outlet
    {
        type            zeroGradient;
    }

    frontAndBack
    {
        type            empty;
    }
}


// ************************************************************************* //


==> Codes/tutorial/0/Ydefault <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       volScalarField;
    location    "0";
    object      Ydefault;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

dimensions      [0 0 0 0 0 0 0];

internalField   uniform 0.0;

boundaryField
{
    inlet
    {
        type            zeroGradient;
    }

    outlet
    {
        type            zeroGradient;
    }


    frontAndBack
    {
        type            empty;
    }
}


// ************************************************************************* //


==> Codes/tutorial/0/p <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       volScalarField;
    location    "0";
    object      p;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

dimensions      [1 -1 -2 0 0 0 0];

internalField   uniform 101325;

boundaryField
{
    inlet
    {
        type            waveTransmissive;
        field           p;
        pis             thermo:psi;
        gamma           1.318654; //cp/cv (inlet)
        fieldInf        101325;
        value           uniform 101325;
    }

    outlet
    {
        type            waveTransmissive;
        field           p;
        pis             thermo:psi;
        gamma           1.272352; // cp/cv (outlet)
        fieldInf        101325;
        value           uniform 101325;
    }

    frontAndBack
    {
        type            empty;
    }
}

// ************************************************************************* //


==> Codes/tutorial/constant/chemistryProperties <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       dictionary;
    location    "constant";
    object      chemistryProperties;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

chemistryType
{
    solver            odePyjac; //ode; odePyjac;
    method	      cemaPyjac; //standard; cemaPyjac;
}

chemistry       on;

initialChemicalTimeStep 1e-8;

odeCoeffs
{
    solver          seulex;
    absTol          1e-08;
    relTol          1e-05;
}

nElements        5;
// ************************************************************************* //


==> Codes/tutorial/constant/thermophysicalProperties <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       dictionary;
    location    "constant";
    object      thermophysicalProperties;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

thermoType
{
    type            hePsiThermo;
    mixture         reactingMixture;
    transport       sutherland;
    thermo          janaf;
    energy          sensibleEnthalpy;
    equationOfState perfectGas;
    specie          specie;
}

inertSpecie N2;

chemistryReader foamChemistryReader;
foamChemistryFile "<constant>/reactionsGRIPyjac";
foamChemistryThermoFile "<constant>/thermo.compressibleGasGRI";

// ************************************************************************* //


==> Codes/tutorial/mechanism/build/Makefile <==
# CMAKE generated file: DO NOT EDIT!
# Generated by "Unix Makefiles" Generator, CMake Version 3.16

# Default target executed when no arguments are given to make.
default_target: all

.PHONY : default_target

# Allow only one "make -f Makefile2" at a time, but pass parallelism.
.NOTPARALLEL:


#=============================================================================
# Special targets provided by cmake.

# Disable implicit rules so canonical targets will work.
.SUFFIXES:


# Remove some rules from gmake that .SUFFIXES does not remove.
SUFFIXES =

.SUFFIXES: .hpux_make_needs_suffix_list


# Suppress display of executed commands.
$(VERBOSE).SILENT:


# A target that is always out of date.
cmake_force:

.PHONY : cmake_force

#=============================================================================
# Set environment variables for the build.

# The shell in which to execute make rules.
SHELL = /bin/sh

# The CMake executable.
CMAKE_COMMAND = /usr/bin/cmake

# The command to remove a file.
RM = /usr/bin/cmake -E remove -f

# Escaping for special characters.
EQUALS = =

# The top-level source directory on which CMake was run.
CMAKE_SOURCE_DIR = /u/34/gadallm1/unix/OpenFOAM/gadallm1-v2006/run/cemaPyjac_tutorial/mechanism

# The top-level build directory on which CMake was run.
CMAKE_BINARY_DIR = /u/34/gadallm1/unix/OpenFOAM/gadallm1-v2006/run/cemaPyjac_tutorial/mechanism/build

#=============================================================================
# Targets provided globally by CMake.

# Special rule for the target install/strip
install/strip: preinstall
	@$(CMAKE_COMMAND) -E cmake_echo_color --switch=$(COLOR) --cyan "Installing the project stripped..."
	/usr/bin/cmake -DCMAKE_INSTALL_DO_STRIP=1 -P cmake_install.cmake
.PHONY : install/strip

# Special rule for the target install/strip
install/strip/fast: preinstall/fast
	@$(CMAKE_COMMAND) -E cmake_echo_color --switch=$(COLOR) --cyan "Installing the project stripped..."
	/usr/bin/cmake -DCMAKE_INSTALL_DO_STRIP=1 -P cmake_install.cmake
.PHONY : install/strip/fast

# Special rule for the target install/local
install/local: preinstall
	@$(CMAKE_COMMAND) -E cmake_echo_color --switch=$(COLOR) --cyan "Installing only the local directory..."
	/usr/bin/cmake -DCMAKE_INSTALL_LOCAL_ONLY=1 -P cmake_install.cmake
.PHONY : install/local

# Special rule for the target install/local
install/local/fast: preinstall/fast
	@$(CMAKE_COMMAND) -E cmake_echo_color --switch=$(COLOR) --cyan "Installing only the local directory..."
	/usr/bin/cmake -DCMAKE_INSTALL_LOCAL_ONLY=1 -P cmake_install.cmake
.PHONY : install/local/fast

# Special rule for the target install
install: preinstall
	@$(CMAKE_COMMAND) -E cmake_echo_color --switch=$(COLOR) --cyan "Install the project..."
	/usr/bin/cmake -P cmake_install.cmake
.PHONY : install

# Special rule for the target install
install/fast: preinstall/fast
	@$(CMAKE_COMMAND) -E cmake_echo_color --switch=$(COLOR) --cyan "Install the project..."
	/usr/bin/cmake -P cmake_install.cmake
.PHONY : install/fast

# Special rule for the target list_install_components
list_install_components:
	@$(CMAKE_COMMAND) -E cmake_echo_color --switch=$(COLOR) --cyan "Available install components are: \"Unspecified\""
.PHONY : list_install_components

# Special rule for the target list_install_components
list_install_components/fast: list_install_components

.PHONY : list_install_components/fast

# Special rule for the target rebuild_cache
rebuild_cache:
	@$(CMAKE_COMMAND) -E cmake_echo_color --switch=$(COLOR) --cyan "Running CMake to regenerate build system..."
	/usr/bin/cmake -S$(CMAKE_SOURCE_DIR) -B$(CMAKE_BINARY_DIR)
.PHONY : rebuild_cache

# Special rule for the target rebuild_cache
rebuild_cache/fast: rebuild_cache

.PHONY : rebuild_cache/fast

# Special rule for the target edit_cache
edit_cache:
	@$(CMAKE_COMMAND) -E cmake_echo_color --switch=$(COLOR) --cyan "No interactive CMake dialog available..."
	/usr/bin/cmake -E echo No\ interactive\ CMake\ dialog\ available.
.PHONY : edit_cache

# Special rule for the target edit_cache
edit_cache/fast: edit_cache

.PHONY : edit_cache/fast

# The main all target
all: cmake_check_build_system
	$(CMAKE_COMMAND) -E cmake_progress_start /u/34/gadallm1/unix/OpenFOAM/gadallm1-v2006/run/cemaPyjac_tutorial/mechanism/build/CMakeFiles /u/34/gadallm1/unix/OpenFOAM/gadallm1-v2006/run/cemaPyjac_tutorial/mechanism/build/CMakeFiles/progress.marks
	$(MAKE) -f CMakeFiles/Makefile2 all
	$(CMAKE_COMMAND) -E cmake_progress_start /u/34/gadallm1/unix/OpenFOAM/gadallm1-v2006/run/cemaPyjac_tutorial/mechanism/build/CMakeFiles 0
.PHONY : all

# The main clean target
clean:
	$(MAKE) -f CMakeFiles/Makefile2 clean
.PHONY : clean

# The main clean target
clean/fast: clean

.PHONY : clean/fast

# Prepare targets for installation.
preinstall: all
	$(MAKE) -f CMakeFiles/Makefile2 preinstall
.PHONY : preinstall

# Prepare targets for installation.
preinstall/fast:
	$(MAKE) -f CMakeFiles/Makefile2 preinstall
.PHONY : preinstall/fast

# clear depends
depend:
	$(CMAKE_COMMAND) -S$(CMAKE_SOURCE_DIR) -B$(CMAKE_BINARY_DIR) --check-build-system CMakeFiles/Makefile.cmake 1
.PHONY : depend

#=============================================================================
# Target rules for targets named c_pyjac

# Build rule for target.
c_pyjac: cmake_check_build_system
	$(MAKE) -f CMakeFiles/Makefile2 c_pyjac
.PHONY : c_pyjac

# fast build rule for target.
c_pyjac/fast:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/build
.PHONY : c_pyjac/fast

out/chem_utils.o: out/chem_utils.c.o

.PHONY : out/chem_utils.o

# target to build an object file
out/chem_utils.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/chem_utils.c.o
.PHONY : out/chem_utils.c.o

out/chem_utils.i: out/chem_utils.c.i

.PHONY : out/chem_utils.i

# target to preprocess a source file
out/chem_utils.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/chem_utils.c.i
.PHONY : out/chem_utils.c.i

out/chem_utils.s: out/chem_utils.c.s

.PHONY : out/chem_utils.s

# target to generate assembly for a file
out/chem_utils.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/chem_utils.c.s
.PHONY : out/chem_utils.c.s

out/dydt.o: out/dydt.c.o

.PHONY : out/dydt.o

# target to build an object file
out/dydt.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/dydt.c.o
.PHONY : out/dydt.c.o

out/dydt.i: out/dydt.c.i

.PHONY : out/dydt.i

# target to preprocess a source file
out/dydt.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/dydt.c.i
.PHONY : out/dydt.c.i

out/dydt.s: out/dydt.c.s

.PHONY : out/dydt.s

# target to generate assembly for a file
out/dydt.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/dydt.c.s
.PHONY : out/dydt.c.s

out/jacob.o: out/jacob.c.o

.PHONY : out/jacob.o

# target to build an object file
out/jacob.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacob.c.o
.PHONY : out/jacob.c.o

out/jacob.i: out/jacob.c.i

.PHONY : out/jacob.i

# target to preprocess a source file
out/jacob.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacob.c.i
.PHONY : out/jacob.c.i

out/jacob.s: out/jacob.c.s

.PHONY : out/jacob.s

# target to generate assembly for a file
out/jacob.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacob.c.s
.PHONY : out/jacob.c.s

out/jacobs/jacob_0.o: out/jacobs/jacob_0.c.o

.PHONY : out/jacobs/jacob_0.o

# target to build an object file
out/jacobs/jacob_0.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_0.c.o
.PHONY : out/jacobs/jacob_0.c.o

out/jacobs/jacob_0.i: out/jacobs/jacob_0.c.i

.PHONY : out/jacobs/jacob_0.i

# target to preprocess a source file
out/jacobs/jacob_0.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_0.c.i
.PHONY : out/jacobs/jacob_0.c.i

out/jacobs/jacob_0.s: out/jacobs/jacob_0.c.s

.PHONY : out/jacobs/jacob_0.s

# target to generate assembly for a file
out/jacobs/jacob_0.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_0.c.s
.PHONY : out/jacobs/jacob_0.c.s

out/jacobs/jacob_1.o: out/jacobs/jacob_1.c.o

.PHONY : out/jacobs/jacob_1.o

# target to build an object file
out/jacobs/jacob_1.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_1.c.o
.PHONY : out/jacobs/jacob_1.c.o

out/jacobs/jacob_1.i: out/jacobs/jacob_1.c.i

.PHONY : out/jacobs/jacob_1.i

# target to preprocess a source file
out/jacobs/jacob_1.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_1.c.i
.PHONY : out/jacobs/jacob_1.c.i

out/jacobs/jacob_1.s: out/jacobs/jacob_1.c.s

.PHONY : out/jacobs/jacob_1.s

# target to generate assembly for a file
out/jacobs/jacob_1.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_1.c.s
.PHONY : out/jacobs/jacob_1.c.s

out/jacobs/jacob_10.o: out/jacobs/jacob_10.c.o

.PHONY : out/jacobs/jacob_10.o

# target to build an object file
out/jacobs/jacob_10.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_10.c.o
.PHONY : out/jacobs/jacob_10.c.o

out/jacobs/jacob_10.i: out/jacobs/jacob_10.c.i

.PHONY : out/jacobs/jacob_10.i

# target to preprocess a source file
out/jacobs/jacob_10.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_10.c.i
.PHONY : out/jacobs/jacob_10.c.i

out/jacobs/jacob_10.s: out/jacobs/jacob_10.c.s

.PHONY : out/jacobs/jacob_10.s

# target to generate assembly for a file
out/jacobs/jacob_10.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_10.c.s
.PHONY : out/jacobs/jacob_10.c.s

out/jacobs/jacob_2.o: out/jacobs/jacob_2.c.o

.PHONY : out/jacobs/jacob_2.o

# target to build an object file
out/jacobs/jacob_2.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_2.c.o
.PHONY : out/jacobs/jacob_2.c.o

out/jacobs/jacob_2.i: out/jacobs/jacob_2.c.i

.PHONY : out/jacobs/jacob_2.i

# target to preprocess a source file
out/jacobs/jacob_2.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_2.c.i
.PHONY : out/jacobs/jacob_2.c.i

out/jacobs/jacob_2.s: out/jacobs/jacob_2.c.s

.PHONY : out/jacobs/jacob_2.s

# target to generate assembly for a file
out/jacobs/jacob_2.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_2.c.s
.PHONY : out/jacobs/jacob_2.c.s

out/jacobs/jacob_3.o: out/jacobs/jacob_3.c.o

.PHONY : out/jacobs/jacob_3.o

# target to build an object file
out/jacobs/jacob_3.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_3.c.o
.PHONY : out/jacobs/jacob_3.c.o

out/jacobs/jacob_3.i: out/jacobs/jacob_3.c.i

.PHONY : out/jacobs/jacob_3.i

# target to preprocess a source file
out/jacobs/jacob_3.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_3.c.i
.PHONY : out/jacobs/jacob_3.c.i

out/jacobs/jacob_3.s: out/jacobs/jacob_3.c.s

.PHONY : out/jacobs/jacob_3.s

# target to generate assembly for a file
out/jacobs/jacob_3.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_3.c.s
.PHONY : out/jacobs/jacob_3.c.s

out/jacobs/jacob_4.o: out/jacobs/jacob_4.c.o

.PHONY : out/jacobs/jacob_4.o

# target to build an object file
out/jacobs/jacob_4.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_4.c.o
.PHONY : out/jacobs/jacob_4.c.o

out/jacobs/jacob_4.i: out/jacobs/jacob_4.c.i

.PHONY : out/jacobs/jacob_4.i

# target to preprocess a source file
out/jacobs/jacob_4.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_4.c.i
.PHONY : out/jacobs/jacob_4.c.i

out/jacobs/jacob_4.s: out/jacobs/jacob_4.c.s

.PHONY : out/jacobs/jacob_4.s

# target to generate assembly for a file
out/jacobs/jacob_4.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_4.c.s
.PHONY : out/jacobs/jacob_4.c.s

out/jacobs/jacob_5.o: out/jacobs/jacob_5.c.o

.PHONY : out/jacobs/jacob_5.o

# target to build an object file
out/jacobs/jacob_5.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_5.c.o
.PHONY : out/jacobs/jacob_5.c.o

out/jacobs/jacob_5.i: out/jacobs/jacob_5.c.i

.PHONY : out/jacobs/jacob_5.i

# target to preprocess a source file
out/jacobs/jacob_5.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_5.c.i
.PHONY : out/jacobs/jacob_5.c.i

out/jacobs/jacob_5.s: out/jacobs/jacob_5.c.s

.PHONY : out/jacobs/jacob_5.s

# target to generate assembly for a file
out/jacobs/jacob_5.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_5.c.s
.PHONY : out/jacobs/jacob_5.c.s

out/jacobs/jacob_6.o: out/jacobs/jacob_6.c.o

.PHONY : out/jacobs/jacob_6.o

# target to build an object file
out/jacobs/jacob_6.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_6.c.o
.PHONY : out/jacobs/jacob_6.c.o

out/jacobs/jacob_6.i: out/jacobs/jacob_6.c.i

.PHONY : out/jacobs/jacob_6.i

# target to preprocess a source file
out/jacobs/jacob_6.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_6.c.i
.PHONY : out/jacobs/jacob_6.c.i

out/jacobs/jacob_6.s: out/jacobs/jacob_6.c.s

.PHONY : out/jacobs/jacob_6.s

# target to generate assembly for a file
out/jacobs/jacob_6.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_6.c.s
.PHONY : out/jacobs/jacob_6.c.s

out/jacobs/jacob_7.o: out/jacobs/jacob_7.c.o

.PHONY : out/jacobs/jacob_7.o

# target to build an object file
out/jacobs/jacob_7.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_7.c.o
.PHONY : out/jacobs/jacob_7.c.o

out/jacobs/jacob_7.i: out/jacobs/jacob_7.c.i

.PHONY : out/jacobs/jacob_7.i

# target to preprocess a source file
out/jacobs/jacob_7.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_7.c.i
.PHONY : out/jacobs/jacob_7.c.i

out/jacobs/jacob_7.s: out/jacobs/jacob_7.c.s

.PHONY : out/jacobs/jacob_7.s

# target to generate assembly for a file
out/jacobs/jacob_7.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_7.c.s
.PHONY : out/jacobs/jacob_7.c.s

out/jacobs/jacob_8.o: out/jacobs/jacob_8.c.o

.PHONY : out/jacobs/jacob_8.o

# target to build an object file
out/jacobs/jacob_8.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_8.c.o
.PHONY : out/jacobs/jacob_8.c.o

out/jacobs/jacob_8.i: out/jacobs/jacob_8.c.i

.PHONY : out/jacobs/jacob_8.i

# target to preprocess a source file
out/jacobs/jacob_8.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_8.c.i
.PHONY : out/jacobs/jacob_8.c.i

out/jacobs/jacob_8.s: out/jacobs/jacob_8.c.s

.PHONY : out/jacobs/jacob_8.s

# target to generate assembly for a file
out/jacobs/jacob_8.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_8.c.s
.PHONY : out/jacobs/jacob_8.c.s

out/jacobs/jacob_9.o: out/jacobs/jacob_9.c.o

.PHONY : out/jacobs/jacob_9.o

# target to build an object file
out/jacobs/jacob_9.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_9.c.o
.PHONY : out/jacobs/jacob_9.c.o

out/jacobs/jacob_9.i: out/jacobs/jacob_9.c.i

.PHONY : out/jacobs/jacob_9.i

# target to preprocess a source file
out/jacobs/jacob_9.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_9.c.i
.PHONY : out/jacobs/jacob_9.c.i

out/jacobs/jacob_9.s: out/jacobs/jacob_9.c.s

.PHONY : out/jacobs/jacob_9.s

# target to generate assembly for a file
out/jacobs/jacob_9.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/jacobs/jacob_9.c.s
.PHONY : out/jacobs/jacob_9.c.s

out/mass_mole.o: out/mass_mole.c.o

.PHONY : out/mass_mole.o

# target to build an object file
out/mass_mole.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/mass_mole.c.o
.PHONY : out/mass_mole.c.o

out/mass_mole.i: out/mass_mole.c.i

.PHONY : out/mass_mole.i

# target to preprocess a source file
out/mass_mole.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/mass_mole.c.i
.PHONY : out/mass_mole.c.i

out/mass_mole.s: out/mass_mole.c.s

.PHONY : out/mass_mole.s

# target to generate assembly for a file
out/mass_mole.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/mass_mole.c.s
.PHONY : out/mass_mole.c.s

out/mechanism.o: out/mechanism.c.o

.PHONY : out/mechanism.o

# target to build an object file
out/mechanism.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/mechanism.c.o
.PHONY : out/mechanism.c.o

out/mechanism.i: out/mechanism.c.i

.PHONY : out/mechanism.i

# target to preprocess a source file
out/mechanism.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/mechanism.c.i
.PHONY : out/mechanism.c.i

out/mechanism.s: out/mechanism.c.s

.PHONY : out/mechanism.s

# target to generate assembly for a file
out/mechanism.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/mechanism.c.s
.PHONY : out/mechanism.c.s

out/rxn_rates.o: out/rxn_rates.c.o

.PHONY : out/rxn_rates.o

# target to build an object file
out/rxn_rates.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/rxn_rates.c.o
.PHONY : out/rxn_rates.c.o

out/rxn_rates.i: out/rxn_rates.c.i

.PHONY : out/rxn_rates.i

# target to preprocess a source file
out/rxn_rates.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/rxn_rates.c.i
.PHONY : out/rxn_rates.c.i

out/rxn_rates.s: out/rxn_rates.c.s

.PHONY : out/rxn_rates.s

# target to generate assembly for a file
out/rxn_rates.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/rxn_rates.c.s
.PHONY : out/rxn_rates.c.s

out/rxn_rates_pres_mod.o: out/rxn_rates_pres_mod.c.o

.PHONY : out/rxn_rates_pres_mod.o

# target to build an object file
out/rxn_rates_pres_mod.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/rxn_rates_pres_mod.c.o
.PHONY : out/rxn_rates_pres_mod.c.o

out/rxn_rates_pres_mod.i: out/rxn_rates_pres_mod.c.i

.PHONY : out/rxn_rates_pres_mod.i

# target to preprocess a source file
out/rxn_rates_pres_mod.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/rxn_rates_pres_mod.c.i
.PHONY : out/rxn_rates_pres_mod.c.i

out/rxn_rates_pres_mod.s: out/rxn_rates_pres_mod.c.s

.PHONY : out/rxn_rates_pres_mod.s

# target to generate assembly for a file
out/rxn_rates_pres_mod.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/rxn_rates_pres_mod.c.s
.PHONY : out/rxn_rates_pres_mod.c.s

out/sparse_multiplier.o: out/sparse_multiplier.c.o

.PHONY : out/sparse_multiplier.o

# target to build an object file
out/sparse_multiplier.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/sparse_multiplier.c.o
.PHONY : out/sparse_multiplier.c.o

out/sparse_multiplier.i: out/sparse_multiplier.c.i

.PHONY : out/sparse_multiplier.i

# target to preprocess a source file
out/sparse_multiplier.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/sparse_multiplier.c.i
.PHONY : out/sparse_multiplier.c.i

out/sparse_multiplier.s: out/sparse_multiplier.c.s

.PHONY : out/sparse_multiplier.s

# target to generate assembly for a file
out/sparse_multiplier.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/sparse_multiplier.c.s
.PHONY : out/sparse_multiplier.c.s

out/spec_rates.o: out/spec_rates.c.o

.PHONY : out/spec_rates.o

# target to build an object file
out/spec_rates.c.o:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/spec_rates.c.o
.PHONY : out/spec_rates.c.o

out/spec_rates.i: out/spec_rates.c.i

.PHONY : out/spec_rates.i

# target to preprocess a source file
out/spec_rates.c.i:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/spec_rates.c.i
.PHONY : out/spec_rates.c.i

out/spec_rates.s: out/spec_rates.c.s

.PHONY : out/spec_rates.s

# target to generate assembly for a file
out/spec_rates.c.s:
	$(MAKE) -f CMakeFiles/c_pyjac.dir/build.make CMakeFiles/c_pyjac.dir/out/spec_rates.c.s
.PHONY : out/spec_rates.c.s

# Help Target
help:
	@echo "The following are some of the valid targets for this Makefile:"
	@echo "... all (the default if no target is provided)"
	@echo "... clean"
	@echo "... depend"
	@echo "... install/strip"
	@echo "... install/local"
	@echo "... install"
	@echo "... list_install_components"
	@echo "... rebuild_cache"
	@echo "... edit_cache"
	@echo "... c_pyjac"
	@echo "... out/chem_utils.o"
	@echo "... out/chem_utils.i"
	@echo "... out/chem_utils.s"
	@echo "... out/dydt.o"
	@echo "... out/dydt.i"
	@echo "... out/dydt.s"
	@echo "... out/jacob.o"
	@echo "... out/jacob.i"
	@echo "... out/jacob.s"
	@echo "... out/jacobs/jacob_0.o"
	@echo "... out/jacobs/jacob_0.i"
	@echo "... out/jacobs/jacob_0.s"
	@echo "... out/jacobs/jacob_1.o"
	@echo "... out/jacobs/jacob_1.i"
	@echo "... out/jacobs/jacob_1.s"
	@echo "... out/jacobs/jacob_10.o"
	@echo "... out/jacobs/jacob_10.i"
	@echo "... out/jacobs/jacob_10.s"
	@echo "... out/jacobs/jacob_2.o"
	@echo "... out/jacobs/jacob_2.i"
	@echo "... out/jacobs/jacob_2.s"
	@echo "... out/jacobs/jacob_3.o"
	@echo "... out/jacobs/jacob_3.i"
	@echo "... out/jacobs/jacob_3.s"
	@echo "... out/jacobs/jacob_4.o"
	@echo "... out/jacobs/jacob_4.i"
	@echo "... out/jacobs/jacob_4.s"
	@echo "... out/jacobs/jacob_5.o"
	@echo "... out/jacobs/jacob_5.i"
	@echo "... out/jacobs/jacob_5.s"
	@echo "... out/jacobs/jacob_6.o"
	@echo "... out/jacobs/jacob_6.i"
	@echo "... out/jacobs/jacob_6.s"
	@echo "... out/jacobs/jacob_7.o"
	@echo "... out/jacobs/jacob_7.i"
	@echo "... out/jacobs/jacob_7.s"
	@echo "... out/jacobs/jacob_8.o"
	@echo "... out/jacobs/jacob_8.i"
	@echo "... out/jacobs/jacob_8.s"
	@echo "... out/jacobs/jacob_9.o"
	@echo "... out/jacobs/jacob_9.i"
	@echo "... out/jacobs/jacob_9.s"
	@echo "... out/mass_mole.o"
	@echo "... out/mass_mole.i"
	@echo "... out/mass_mole.s"
	@echo "... out/mechanism.o"
	@echo "... out/mechanism.i"
	@echo "... out/mechanism.s"
	@echo "... out/rxn_rates.o"
	@echo "... out/rxn_rates.i"
	@echo "... out/rxn_rates.s"
	@echo "... out/rxn_rates_pres_mod.o"
	@echo "... out/rxn_rates_pres_mod.i"
	@echo "... out/rxn_rates_pres_mod.s"
	@echo "... out/sparse_multiplier.o"
	@echo "... out/sparse_multiplier.i"
	@echo "... out/sparse_multiplier.s"
	@echo "... out/spec_rates.o"
	@echo "... out/spec_rates.i"
	@echo "... out/spec_rates.s"
.PHONY : help



#=============================================================================
# Special targets to cleanup operation of make.

# Special rule to run CMake to check the build system integrity.
# No rule that depends on this can have commands that come from listfiles
# because they might be regenerated.
cmake_check_build_system:
	$(CMAKE_COMMAND) -S$(CMAKE_SOURCE_DIR) -B$(CMAKE_BINARY_DIR) --check-build-system CMakeFiles/Makefile.cmake 0
.PHONY : cmake_check_build_system



==> Codes/tutorial/system/blockMeshDict <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       dictionary;
    object      blockMeshDict;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

scale   0.01;

vertices
(
    (0          0       0)
    (2.0        0       0)
    (2.0        0.25    0)
    (0          0.25    0)
    (0          0       0.25)
    (2.0        0       0.25)
    (2.0        0.25    0.25)
    (0          0.25    0.25)
);

blocks
(
    hex (0 1 2 3 4 5 6 7) (1350 1 1) simpleGrading (1 1 1)
);

edges
(
);

boundary
(
    inlet
    {
        type patch;
        faces
        (
           (4 7 3 0)
        );
    }
    outlet
    {
        type patch;
        faces
        (
            (1 2 6 5)
        );
    }

    frontAndBack
    {
        type empty;
        faces
        (
            (0 3 2 1)
            (4 5 6 7)
            (7 6 2 3)
            (1 0 4 5)
        );
    }
);

mergePatchPairs
(
);

// ************************************************************************* //


==> Codes/tutorial/system/controlDict <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       dictionary;
    location    "system";
    object      controlDict;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

application     reactingFoam;

startFrom       startTime;

startTime       0;

stopAt          endTime;

endTime         0.002;

deltaT          1e-8;

writeControl    adjustableRunTime;

writeInterval   1e-04;

purgeWrite      0;

writeFormat     ascii;

writePrecision  6;

writeCompression off;

timeFormat      general;

timePrecision   6;

runTimeModifiable true;

adjustTimeStep  yes;

maxCo           0.3;

libs (
      "libcemaPyjacChemistryModel.so"
      "$FOAM_CASE/constant/libc_pyjac.so"
     );

// ************************************************************************* //


==> Codes/tutorial/system/fvSolution <==
/*--------------------------------*- C++ -*----------------------------------*\
| =========                 |                                                 |
| \\      /  F ield         | OpenFOAM: The Open Source CFD Toolbox           |
|  \\    /   O peration     | Version:  v2006                                 |
|   \\  /    A nd           | Website:  www.openfoam.com                      |
|    \\/     M anipulation  |                                                 |
\*---------------------------------------------------------------------------*/
FoamFile
{
    version     2.0;
    format      ascii;
    class       dictionary;
    location    "system";
    object      fvSolution;
}
// * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * //

solvers
{
    rho
    {
        solver           PCG;
        preconditioner   DIC;
        tolerance        1e-8;
        relTol           0.005;
    }

    rhoFinal
    {
        $rho;
        tolerance 1e-8;
        relTol           0.0;
    }
    p
    {
        solver           PCG;
        preconditioner   DIC;
        tolerance        1e-8;
        relTol           0.005;
    }

    pFinal
    {
        $p;
        tolerance 1e-8;
        relTol           0.0;
    }

    "(U|h|k|epsilon)"
    {
        solver          PBiCGStab;
        preconditioner  DILU;
        tolerance       1e-7;
        relTol          0.005;
    }

    "(U|h|k|epsilon)Final"
    {
        $U;
        relTol          0;
    }

    Yi
    {
        $hFinal;
    }

    YiFinal
    {
        $Yi;
    }

}

PIMPLE
{
    momentumPredictor no;
    nOuterCorrectors  3;
    nCorrectors     4;
    nNonOrthogonalCorrectors 0;
}

// ************************************************************************* //


==> Includes/Chapters/Codes.tex <==
\chapter{Including codes}

\section{\texttt{verbatim} environment}

You should use the \verb|verbatim| style when you want to refer to OpenFOAM commands, keywords, addresses, etc. You can either use the inline command \verb|\verb|, or the the full \verb|verbatim| environment. For instance see the following paragraph. 

\subsection{\texttt{verbatim} example}
Copy the \verb|pitzDaily| case in your \verb|run| directory with this command:
\begin{verbatim}
cp -r  $FOAM_TUTORIALS/incompressible/simpleFoam/pitzDaily
\end{verbatim}
You should perform your simulations with the following turbulence models:
\begin{itemize}
	\item Spalart Allmaras (\verb|SpalartAllmaras|)
	\item Launder-Sharma $k-\varepsilon$  (\verb|LaunderSharmaKE|)
	\item $k-\omega$ SST  (\verb|kOmegaSST|)
	\item $k-\varepsilon-\phi-f$  (\verb|kEpsilonPhitF|)
\end{itemize}

The second-order upwind differencing scheme (\verb|linearUpwind|) should be used for discretization of the convective term in momentum transport equation while other convective terms should be discretized using the limited linear differencing scheme (\verb|limitedLinear|). In addition, The gradient and diffusion terms must be discretized using the central differencing scheme.


\section{Including a piece of code}
You should use the \verb|lstlisting| environment to include a piece of code in your text. Two customized \verb|lstlisting| styles are available in this report template, i.e., \verb|cpp| and \verb|OpenFOAMDict|, that should be used for your C++ codes and OpenFOAM dictionaries, respectively. If you have a code in other languages (e.g. Python), you can define the a new \verb|lstlisting| style. See the following example. 

\begin{lstlisting}[style=cpp,title=A piece of code,captionpos=t]
# include <iostream>

int main()
{
	//This is a comment!
	std::cout << "Hello, world!\n"; 
}
\end{lstlisting}

\section{Including a dictionary from source file}
If you want to include the content of an ASCII file in the document you do not need copy the contents into the text. You can just simply use \verb|\lstinputlisting| command to include your code. Here is an example of an OpenFOAM dictionary file.

\lstinputlisting[style=OpenFOAMDict,title=\texttt{controlDict},captionpos=t]{Codes/controlDict}

Note that you should avoid including long code listings that do not have any descriptions. They can be put in the appendix, if they need to be part of the document. However, you can insert and describe a part of a code into your document. For instance, the following example shows the PISO corrector loop in the \verb|icoFoam| solver. Note the \verb|linerange| and \verb|firstnumber| commands.

\lstinputlisting[style=cpp, title=The PISO corrector loop in the \texttt{icoFoam} solver,captionpos=t, linerange={116-156},firstnumber=116]{Codes/icoFoam.C}


==> Includes/Chapters/FigsTabs.tex <==
\chapter{Figures and tables}

\section{Figures}
All figures should be positioned at a good position near to corresponding text. The \verb|figure| environment must be used to create figures. You are highly encouraged to create publication quality \emph{vector} pictures. Here is an example of creating a figure and then referring to it.

Figure~\ref{fig:CoverPic} illustrates the development of streamwise velocity in the planar asymmetric diffuser. In this figure, the numerical results are validated with the experimental data. An example of \verb|subfigure| environment is also shown in Figure~\ref{fig:Cf}.
 
\begin{figure}[!htbp]
	\centering
	\includegraphics[width=1\textwidth]{Figures/CoverPic}
	\caption{Development of streamwise velocity in the planar asymmetric diffuser}
	\label{fig:CoverPic}
\end{figure} 



\begin{figure}[!hbpt]
	\centering
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{Figures/cf_lowerWall}
		\caption{Lower wall}
		\label{fig:Cf_L}
	\end{subfigure}
	\hspace{0.02\textwidth}
	\begin{subfigure}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=1\textwidth]{Figures/cf_upperWall}
		\caption{Upper wall}
		\label{fig:Cf_U}
	\end{subfigure}
	\caption{Skin friction coefficient on both walls}
	\label{fig:Cf}
\end{figure}



\section{Tables}

A table example is shown in Table~\ref{tab:exampleTable}. You can use online latex table generator tools to produce more advanced tables (e.g. \href{https://www.tablesgenerator.com/}{www.tablesgenerator.com}).


\begin{table}[t]
	\caption{Table caption}
	\label{tab:exampleTable}
    \centering
	\begin{tabular}{l l l}
		\hline
		Example & Time & Cost \\
		\hline
		1 & 12.5 & \$1,000 \\
		2 & 24 & \$2,000 \\
		3 & 36 & \$4,000 \\
		4 & 48 & \$8,000 \\
		\hline
	\end{tabular}
\end{table}

==> Includes/Chapters/Math.tex <==
\chapter{Typesetting mathematical formulations}

\LaTeX\ is undoubtedly the most powerful document preparation system when it comes to typesetting mathematical formulations. In this chapter some examples of mathematical equations in \LaTeX\ are presented. For more information please see Chapter 3 of \cite{notSoShort}.



\section{Proper mathematical typesetting}

\subsection{Variables}
One general rule in the correct mathematical typesetting is that anything that represents a variable (for example, $U$ for a velocity) should appear in \emph{italic} format, and everything else should be set in \emph{roman} (non-italic) type. Please note, in \LaTeX, both inline equation and equation environment automatically italicize all variables. Therefore, if you have a word inside an equation, you should manually set it roman. One exception to this rule is with multiple-letter symbols. In order to avoid interpreting these numbers as the multiplication of two variables, they could be typeset upright. For instance, dimensionless numbers in fluid mechanics such as Reynolds and Prandtl number could be set roman ($\mathrm{Re}$, $\mathrm{Pr}$).

Operators, such as $\cos$ and $\log$ (representing the cosine and logarithm functions) are not variables and should therefore be set roman. For vectors, matrices and tensors, it is recommended to set the variable itself in boldface (excluding any associated subscripts or superscripts).


\subsection{Subscripts and superscripts}
The same rule applies to subscription and superscription. See the following examples.
\begin{itemize}
    \item $U_\mathrm{i}$: if ``i" stands for ``inlet" which is a word.
    \item $U_i$: if ``$i$" is a variable denoting $i$th index.
\end{itemize}

\subsection{Derivative and integral}
The differentiation operator, $\mathrm{d}$, in derivative or integral is not a variable and therefore should be upright, not italics. It is also advisable to use spacing inside the integral to make it more clear. See the following examples.

\begin{equation}
    f'(x) = \frac{\mathrm{d}f(x)}{\mathrm{d}x}
\end{equation}

\begin{equation}
    \int_a^b \! f(x) \, \mathrm{d}x = F(x) \Big|_a^b
\end{equation}

Note the \verb|\!| and \verb|\,| in the integral command for proper spacing.


\subsection{Physical units}
All physical units must be set roman. As an example, $p_\mathrm{atm}=101$~kPa is correct and $p_\mathrm{atm}=101~kPa$ is incorrect.



\section{Example}

The governing equations of the mean fluid flow and Launder-Sharma $k-\varepsilon$ turbulence model are presented in this section.

\subsection{Navier-Stokes equations}
For a statistically stationary incompressible turbulent flow, the time-averaged equations of mass and momentum in tensorial form are written as:
\begin{equation}
\frac{\partial U_j}{\partial x_j}=0,
\label{eqn:Continuity}
\end{equation}
\begin{equation}
\frac{\partial (U_i U_j)}{\partial x_j}=\frac{-1}{\rho }\frac{\partial p}{\partial x_i}+\frac{\partial }{\partial x_j}\left( \nu \frac{\partial U_i}{\partial x_j}-\overline{u_i u_j} \right),
\label{eqn:RANS}
\end{equation}
where $-\rho \overline{{{u}_{i}}{{u}_{j}}}$ is the unknown Reynolds stress tensor and the system of equations cannot be solved unless this term is identified. 


\subsection{Launder-Sharma \texorpdfstring{$k-\varepsilon$}{k-e} model}
In the $k-\varepsilon$ model, turbulent stresses are obtained using the Boussinesq (eddy-viscosity) hypothesis
\begin{equation}
\overline{{{u}_{i}}{{u}_{j}}}=-{{\nu }_{t}}\left(\frac{\partial {{U}_{i}}}{\partial {{x}_{j}}}+\frac{\partial {{U}_{j}}}{\partial {{x}_{i}}}\right)+\frac{2}{3}k{{\delta }_{ij}},
\label{eqn:Boussinesq}
\end{equation}
where the turbulent viscosity is calculated via
\begin{equation}
{{\nu }_{t}}={{C}_{\mu }}{{f}_{\mu }}\frac{{{k}^{2}}}{\varepsilon }
\label{eqn:k_eps_nut}.
\end{equation}
To obtain $\nu_t$, transport equations for the turbulent kinetic energy $k$, and homogeneous dissipation rate $\tilde{\varepsilon}$ are solved. The transport equation for the turbulent kinetic energy is written as
\begin{equation}
\frac{\partial }{\partial {{x}_{j}}}({{U}_{j}}k)=\frac{\partial }{\partial {{x}_{j}}}\left[ \left( \nu +\frac{{{\nu }_{t}}}{{{\sigma }_{k}}} \right)\frac{\partial k}{\partial {{x}_{j}}} \right]+{{P}_{k}}-\tilde{\varepsilon }-2\nu {{\left( \frac{\partial \sqrt{k}}{\partial {{x}_{j}}} \right)}^{2}}.
\label{eqn:k_eps_k}
\end{equation}
Also the homogeneous dissipation rate of the turbulent kinetic energy is obtained by solving the equation
\begin{equation}
\frac{\partial }{\partial {{x}_{j}}}({{U}_{j}}\tilde{\varepsilon })=\frac{\partial }{\partial {{x}_{j}}}\left[ \left( \nu +\frac{{{\nu }_{t}}}{{{\sigma }_{\varepsilon }}} \right)\frac{\partial \tilde{\varepsilon }}{\partial {{x}_{j}}} \right]+{{C}_{\varepsilon 1}}\frac{{\tilde{\varepsilon }}}{{{\sigma }_{\varepsilon }}}{{P}_{k}}-{{C}_{\varepsilon 2}}{{f}_{2}}\frac{{{{\tilde{\varepsilon }}}^{2}}}{k}+E.
\label{eqn:k_eps_eps}
\end{equation}

Here is an example of how to refer to the Eq.~\eqref{eqn:RANS}.







\subsection{Some advanced equations}

\begin{equation}
y\equiv\mathcal{U}(\boldsymbol{x};{\boldsymbol{\xi}}) \simeq {\mathcal{U}}_{\mathrm{PC}}(\boldsymbol{x};{\boldsymbol{\xi}}) = \sum_{0 \leqslant \left| \boldsymbol{\alpha} \right| \leqslant p} \!
u_{\boldsymbol{\alpha}}({\boldsymbol{x}})\boldsymbol{\psi}_{\boldsymbol{\alpha}}({\boldsymbol{\xi}}), \quad \left| \boldsymbol{\alpha} \right|=\sum_{i=1}^d \alpha_i.
\label{eqn:PCE_Main2}
\end{equation}

\begin{equation}
u_{\boldsymbol{\alpha}}(\boldsymbol{x})=\frac{1}{\langle \boldsymbol{\psi}_{\boldsymbol{\alpha}}^2(\boldsymbol{\xi}) \rangle}\int_{\Omega} \! \mathcal{U}(\boldsymbol{x},\boldsymbol{\xi}) \boldsymbol{\psi}_{\boldsymbol{\alpha}}(\boldsymbol{\xi}){\boldsymbol{f}(\boldsymbol{\xi})} \mathrm{d}\boldsymbol{\xi}.
\label{eqn:PCE_Projection1}
\end{equation}


\begin{equation}
\mathscr{I}_{i_1,\cdots,i_s}=\left\{ \boldsymbol{\alpha}:\begin{matrix} 
\alpha_k>0 \quad \forall k=1,\cdots,n, \quad k \in (i_1,\cdots,i_s) \\ 
\alpha_j=0 \quad \forall k=1,\cdots,n, \quad k \notin (i_1,\cdots,i_s) \\ 
\end{matrix} \right\}.
\end{equation}



\begin{equation}
\begin{split}
\mathrm{Var}[u] &= \mathbb{E} \left[  \left( u - \mathbb{E}[u] \right)^2  \right] =
\mathbb{E} \left[  \left( \left(  \sum_{k=0}^P u_k \psi_k  \right) - u_0 \right)^2  \right] \\
& = \mathbb{E} \left[  \left(  \sum_{k=1}^P u_k \psi_k  \right)^2  \right] = 
\sum_{k=1}^P u_k^2 \mathbb{E}[\psi_k^2] = \sum_{k=1}^P u_k^2 (k!)^2
\end{split}
\end{equation}



\begin{equation}
\begin{split}
\mathcal{U}(\boldsymbol{x},\boldsymbol{\xi})  = u_0 & + \sum_{i=1}^{n}\sum_{\boldsymbol{\alpha} \in \mathscr{I}_i} u_{\boldsymbol{\alpha}}(x_i) \boldsymbol{\psi}_{\boldsymbol{\alpha}}(\xi_i) \\
& + \sum_{1 \le {i_1}<{i_2} \le n}\sum_{\boldsymbol{\alpha} \in \mathscr{I}_{i_1,i_2}} u_{\boldsymbol{\alpha}}(x_{i_1},x_{i_2}) \boldsymbol{\psi}_{\boldsymbol{\alpha}}(\xi_{i_1},\xi_{i_2}) +\cdots \\
& + \sum_{1\le {i_1}<\cdots<{i_s}\le n} \sum_{\boldsymbol{\alpha} \in \mathscr{I}_{i_1,\cdots,i_s}} u_{\boldsymbol{\alpha}}(x_{i_1},\cdots,x_{i_s}) \boldsymbol{\psi}_{\boldsymbol{\alpha}}(\xi_{i_1},\cdots,\xi_{i_s})  +\cdots \\
& + \sum_{\boldsymbol{\alpha} \in \mathscr{I}_{1,\cdots,n}} u_{\boldsymbol{\alpha}}(x_1,\cdots,x_n) \boldsymbol{\psi}_{\boldsymbol{\alpha}}(\xi_1,\cdots,\xi_n).
\end{split}
\label{eqn:Sobol_Decomp_of_PCE}
\end{equation}

==> Includes/Chapters/Nom.tex <==
\chapter{Nomenclature and Index}

This chapter describes how to create Nomenclature and Index in \LaTeX. Please note that having Nomenclature and Index sections in your report is recommended, as it can be very informative and helpful for the future readers of your report.

\section{Nomenclature}

All the acronyms, symbols, subscripts, and superscripts should be described in the Nomenclature section. Please follow the presented examples in this template in the \verb|Includes/Nomenclature.tex| file. The nomenclature list is created by means of the \verb|nomencl| and \verb|siunitx| packages.

You can see that there are predefined subgroups in the list. These subgroups are presented in Table \ref{tab:NomSubgroups}. If you need to define extra subgroups you can manipulate the \emph{Nomenclature definition} section of the \verb|Includes/Settings.tex| file. The list is automatically presented in the alphabetical order.

\begin{table}[!h]
	\caption{Nomenclature subgroups}
	\label{tab:NomSubgroups}
    \centering
    \begin{tabular}{c c}
		\hline
		Prefix & Group \\
		\hline
		A & Acronyms \\
		E & English \\
		G & Greek \\
		S & Superscripts \\
		U & Subscripts \\
		X & Other Symbols \\
		\hline
	\end{tabular}
\end{table}

\section{Index}
An index is a list of words or phrases (``headings") and associated pointers (``locators") to where useful material relating to that heading can be found in a document or collection of documents \cite{IndexWiki}. The index list is created using the \verb|imakeidx| package. This document has the index at the end (please have a look).

In this example (see \LaTeX~source code of this paragraph) several keywords\index{keywords} will be used which are important and deserve to appear in the index\index{index}. Terms like OpenFOAM\index{OpenFOAM}, project\index{project}, report\index{report} and some others\index{others} will also show up.


There is no need to bother about the index keywords when writing the document. After you are finished with the report, you may decide which index keywords you want to use, and use search and replace to create the index. For instance, if you wish to index the keyword \verb|turbulence|, you may search for all of the instances of that keyword and \emph{manually accept the replacement of them} with \verb|turbulence\index{turbulence}|. Just make sure that you do not replace your keywords inside verbatim mode, since then it will not work properly! Instead, put the \verb|\index{}| just outside the verbatim mode. That is why you should manually accept every replacement rather than to automatically accept all of them. Some typical keywords would be standard OpenFOAM solvers, utilities, libraries, classes, etc., as well as your own developments. Quite often you may be using verbatim mode for OpenFOAM names. Again, make sure that the \verb|\index{}| ends up outside the verbatim mode!

==> Includes/Chapters/Refs.tex <==
\chapter{References}

the {\sc Bib}\TeX\ tool is employed for citing references and creating bibliography. The referencing style is \verb|ieeetr|. The references are kept in the \verb|Bibliography.bib| file and the \verb|\cite| command should be use for the citation. Here is an example of single citation \cite{einstein} and multiple citations \cite{latexcompanion,knuthwebsite}.


==> nomencl/Makefile <==

PACKAGE=nomencl

SAMPLES = sample01.tex sample02.tex sample03.tex sample04.tex sample05.tex 

CFG = sample04.cfg sample05.cfg sample06.cfg


SAMPLEPDF = ${SAMPLES:%.tex=%.pdf}

PDF = $(PACKAGE).pdf ${SAMPLEPDF}

all:  ${PDF} ${SAMPLES} ${CFG} ${PACKAGE}.sty


%.sty:  %.ins %.dtx
	pdflatex $*.ins

sample%.tex:  nomencl.ins nomencl.sty
	pdflatex nomencl.ins

sample%.cfg: nomencl.ins nomencl.dtx
	pdflatex nomencl.ins


%.pdf:  %.dtx ${PACKAGE}.sty 
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


sample%.pdf: sample%.tex ${CFG} ${PACKAGE}.sty
	pdflatex sample$*.tex
	makeindex sample$*.nlo -s nomencl.ist -o sample$*.nls
	pdflatex sample$*.tex
	pdflatex sample$*.tex



clean:
	$(RM)  ${PACKAGE}.sty *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi *.drv *.ist \
	*.nlo *.nls ${SAMPLES} ${CFG}

distclean: clean
	$(RM) $(PDF) 

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

.PRECIOUS: ${SAMPLES} ${CFG}

